Show Me More Details: Discovering Hierarchies of Procedures from Semi-structured Web Data

Procedures are inherently hierarchical. To "make videos", one may need to "purchase a camera", which in turn may require one to "set a budget". While such hierarchical knowledge is critical for reasoning about complex procedures, most existing work has treated procedures as shallow structures without modeling the parent-child relation. In this work, we attempt to construct an open-domain hierarchical knowledge-base (KB) of procedures based on wikiHow, a website containing more than 110k instructional articles, each documenting the steps to carry out a complex procedure. To this end, we develop a simple and efficient method that links steps (e.g., "purchase a camera") in an article to other articles with similar goals (e.g., "how to choose a camera"), recursively constructing the KB. Our method significantly outperforms several strong baselines according to automatic evaluation, human judgment, and application to downstream tasks such as instructional video retrieval. A demo with partial data can be found at https://wikihow-hierarchy.github.io. The code and the data are at https://github.com/shuyanzhou/wikihow_hierarchy.

==> old_table_intrinsic_case.tex <==
\begin{table}[t]\small
  \centering
  \begin{tabular}{l|ll}
  \toprule
  \multirow{4}{*}{\textbf{C1}} & \textit{q} & Eject your external hard drive \\
  & \textit{p} & Eject an External Hard Drive \\
  & \textit{gt} & Unmount a Drive \\
  & \textit{g} & Back Up a Mac Without Time Machine \\
  \midrule
  \multirow{4}{*}{\textbf{C2}} & \textit{q} & Promote your profile \\
  & \textit{p} & Improve Your Profile \\
  & \textit{gt} & Promote Your Instagram \\
  & \textit{g} & Get Followers on Instagram Fast \\
  \midrule
  \multirow{4}{*}{\textbf{C3}} & \textit{q} & Turn off FileVault \\
  & \textit{p} & Encrypt a Mac Hard Drive with FileVault 2 \\
  & \textit{gt} & Turn Off Automatic Encryption on a Mac \\
  & \textit{g} & Back Up a Mac Without Time Machine \\
  \midrule
  \multirow{4}{*}{\textbf{C4}} & \textit{q} & Wash your beard weekly to preserve natural oils \\
  & \textit{p} & Make Natural Essential Oils \\
  & \textit{gt} & Clean a Beard \\
  & \textit{g} & Straighten Beard Hairs \\
  \bottomrule
  
  \end{tabular}
  \caption{The main failure modes of the candidate retrieval model (\textsc{SP}). \textit{q}: the query step; \textit{p}: the top-1 prediction of the retrieval model; \textit{gt}: the ground-truth linked goal of the query step; \textit{g}: the goal of the query step. }
  \label{tab:intrinsic_case}
\end{table}

==> table_vir_example_v1.tex <==
\begin{table*}[t]
    \centering\small
    \begin{tabular}{l|l|l|l}
    \toprule
    Goal & $\textsc{Fil-l}_{1}$ &  $\textsc{Fil-l}_{2}$ & Key Moments
    \\
\midrule
Stain & NaN & (1) Purchase some stain colors to test & [1] Removing doors \\
cabinet &  & (2) Unscrew the cabinet from the wall \textcolor{blue}{[1]} & [2] Sanding the font \\
 &  & (3) Ventilate the room & [3] Top coat \\
 &  & (4) Apply the first coat \textcolor{blue}{[3]} & [4] Finished look \\
\midrule
Touch & (1) Purchase the correct color & (1)(2) of $\textsc{Fil-l}_{1}$ & [1] Letting it dry for around \\
up & touch up paint & (2) Clean the area around the scratch \textcolor{blue}{[2]} & ten minutes \\
scratches & (2) Choose the right conditions & (3) Apply a thin line of touch up & [2] Cleaned up the area with \\
on & to repair it & paint to the scratch using a fine brush & a microfiber towel \\
your & (3) Add a coat of & (4) Buy the abrasive that's best for your & [3] Cleaned the area with water \\
car & paint to the scratch & project & and a microfiber towel \\
 &  & (5) Dry the vehicle with fresh towels \textcolor{blue}{[3,4]} & [4] Wiped it off with a \\
 &  &  & clean microfiber\\
     \bottomrule
    \end{tabular}
        \caption{The resulted $\textsc{Fil-l}_{1}$, $\textsc{Fil-l}_{2}$ queries and the key moments for two goals. The two key moments are taken from Youtube video \href{https://www.youtube.com/watch?v=h9k0T25_NxA}{\texttt{h9k0T25\_NxA}} and \href{https://www.youtube.com/watch?v=-EiAN6oa_oY}{\texttt{EiAN6oa\_oY}}. \textcolor{blue}{[i]} means that the automatically extracted step share the similar semantic with the $i$-th key moment. }
    \label{tab:vir_case}
\end{table*}
